Reflect-RL: Two-Player Online RL Fine-Tuning for LMs

As language models (LMs) demonstrate their capabilities in various fields, their application to tasks requiring multi-round interactions has become increasingly popular. These tasks usually have complex dynamics, so supervised fine-tuning (SFT) on a limited offline dataset does not yield good performance. However, only a few works attempted to directly train the LMs within interactive decision-making environments. We aim to create an effective approach to fine-tune LMs with online reinforcement learning (RL) in these environments. We propose Reflect-RL, a two-player system to fine-tune an LM using SFT and online RL, where a frozen reflection model (player) assists the policy model (player). To generate data for the warm-up SFT stage, we use negative example generation to enhance the error-correction ability of the reflection model. Furthermore, we designed single-prompt action enumeration and applied curriculum learning to allow the policy model to learn more efficiently. Empirically, we verify that Reflect-RL outperforms SFT and online RL without reflection. Testing results indicate GPT-2 XL 1.56B fine-tuned with Reflect-RL outperforms larger open-source LMs, such as Mistral 7B. The benchmarks, dataset, and code involved in this work are publicly available: https://github.com/zhourunlong/Reflect-RL.

==> fig_tex/ae_rst_old.tex <==
518_rl_finetune,zhou_531,zhou_536,step
0.3018867924528302,0.4056603773584906,0.42924528301886794,0
0.28809523809523807,0.35714285714285715,0.5142857142857142,100
0.3142857142857143,0.41904761904761906,0.5190476190476191,200
0.3119047619047619,0.3761904761904762,0.45714285714285713,300
0.26904761904761904,0.43333333333333335,0.3880952380952381,400
0.2761904761904762,0.4380952380952381,0.48333333333333334,500
0.23333333333333334,0.4642857142857143,0.5261904761904762,600
0.2976190476190476,0.44285714285714284,0.45,700
0.2714285714285714,0.4261904761904762,0.5071428571428571,800
0.30714285714285716,0.4857142857142857,0.4928571428571429,900
0.33095238095238094,0.45,0.5142857142857142,1000
0.36666666666666664,0.45476190476190476,0.5357142857142857,1100
0.3738095238095238,0.44761904761904764,0.5285714285714286,1200
0.3904761904761905,0.5119047619047619,0.5380952380952381,1300
0.42857142857142855,0.5261904761904762,0.5761904761904761,1400
0.3738095238095238,0.4642857142857143,0.48095238095238096,1500
,0.4261904761904762,0.5261904761904762,1600
,0.40714285714285714,0.4595238095238095,1700
,0.4,0.4642857142857143,1800
,0.5142857142857142,0.45476190476190476,1900
,0.5261904761904762,0.5047619047619047,2000
,0.5428571428571428,0.4642857142857143,2100
,0.5666666666666667,0.5404761904761904,2200
,0.5357142857142857,0.5452380952380952,2300
,0.5261904761904762,0.55,2400
,0.5857142857142857,0.5238095238095238,2500
,0.55,0.49523809523809526,2600
,0.5119047619047619,0.5595238095238095,2700
,0.5619047619047619,0.5404761904761904,2800
,0.5404761904761904,0.5547619047619048,2900
,0.5380952380952381,0.5023809523809524,3000
,0.5619047619047619,0.49047619047619045,3100
,0.4666666666666667,0.4642857142857143,3200
,0.5476190476190477,0.5166666666666667,3300
,0.530952380952381,0.5619047619047619,3400
,0.5452380952380952,0.4857142857142857,3500
,0.5142857142857142,0.5404761904761904,3600
,0.530952380952381,0.5761904761904761,3700
,0.4595238095238095,0.5642857142857143,3800
,0.5166666666666667,0.5285714285714286,3900
,0.5095238095238095,0.5333333333333333,4000
,0.4666666666666667,0.5547619047619048,4100
,0.5642857142857143,0.580952380952381,4200
,0.5404761904761904,0.55,4300
,0.5404761904761904,0.5595238095238095,4400
,0.5380952380952381,0.5761904761904761,4500
,0.5190476190476191,0.530952380952381,4600
,0.5238095238095238,0.5928571428571429,4700
,0.6142857142857143,0.55,4800
,0.5928571428571429,0.5761904761904761,4900


==> fig_tex/table_file_search_result.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|l|l}
\toprule
\textbf{Method}                  & \textbf{Backbone Model} & \textbf{Performance} \\ 
\midrule
\multirow{3}{*}{RAG}             & llama 7B                & 70                   \\ \cline{2-3} 
                                 & gpt-3.5-turbo           & 90                   \\ \cline{2-3} 
                                 & gpt-4                   & 92                   \\ \hline
\multirow{3}{*}{Agentic Search}  & llama 7B                & 70                   \\ \cline{2-3} 
                                 & gpt-3.5-turbo           & 80                   \\ \cline{2-3} 
                                 & gpt-4                   & 90                   \\ \hline
\multirow{2}{*}{Agentic Search MDP} & gpt-3.5-turbo       & 90                   \\ \cline{2-3} 
                                 & gpt-4                   & 90                   \\ \hline
RLFT                             & llama 7B                & 90                   \\ 
\bottomrule
\end{tabular}
\caption{\beibin{Finish the experiments} File search experiment results}
\label{table:methods_models}
\end{table}

==> rst_details.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{c|l|cc|cc|c}
\toprule
& \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\autoexplore} 
& \multicolumn{2}{c|}{\taxi}  & \multirow{2}{*}{\alfw} \\ 
&    & Depth 1 &  Depth 2 & Pickup & + Dropoff & \\ \hline
% \midrule
% & Random &  &  &  2\% & 0\% & \\
\midrule
 \multirow{4}{*}{OSS}
& Mistral 7B &          &  &  & 0\%  & 0\% \\
& Llama2 7B-chat &      &   & 3\% & 0\% & 0\% \\
& Orca-2 7B & &   &   & 0\%  & \\
& QWEN 14B &          &     & 5\% & 0\%  & \\
\midrule
 \multirow{2}{*}{Commercial}
& GPT-3.5-turbo    &       &  &  4\%  & 0\%   & 6\% \\
& GPT-4   &    &   & 18\%& 0\%  & 84\% \\
\midrule
\rlft (Ours)
& GPT-2-xl 1.56B & 36\$ & 17\% &  58\% & 29\%  & 74\% \\
\bottomrule
\end{tabular}
\caption{Testing performance for $100$ random testing runs. We have included ReAct and memory-mechanism to improve the performance. The GPT models are in version 1106.
GPT-4 might be contaminated with the Alfworld dataset.}
\label{table:all-rst}
\end{table*}

